Label Dependent Deep Variational Paraphrase Generation

Generating paraphrases that are lexically similar but semantically different is a challenging task. Paraphrases of this form can be used to augment data sets for various NLP tasks such as machine reading comprehension and question answering with non-trivial negative examples. In this article, we propose a deep variational model to generate paraphrases conditioned on a label that specifies whether the paraphrases are semantically related or not. We also present new training recipes and KL regularization techniques that improve the performance of variational paraphrasing models. Our proposed model demonstrates promising results in enhancing the generative power of the model by employing label-dependent generation on paraphrasing datasets.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> relatedWorks.tex <==
\section{Related Work}\label{sec:relw}


==> review.tex <==
These are my thoughts and suggestions about the reviews. --Tommy

Reviewer 1 comments:
\begin{quote}
    Writing: Needs major work. There are 3.5 pages of introduction and unnecessary background on submodular functions and two paragraphs in sec 3.2 of what the method proposed in this paper does. Only mentioning what the submodular function is, and may be a couple of references for it should have been enough. Proposition 1 is redundant, just mentioning the result in a single sentence is more than enough. I do not see the benefit of talking about a substantial subset of the submodular literature. The intro itself needs major revisions to be readable, there are a lot of holes. e.g. what is "unfolding" of the greedy algorithm that the  authors refer to?  Use of \tau in f() should be explicitly written as an equation, so the reader doesn’t have to look at the paper by Jang et al to know that the exact expression is used in the training. The experimental task itself could have been explained better. What is  the DeepEncoder architecture? Why was it used as a baseline? Why cant diversity arguments not be made by easily altering the DeepEncoder cost function? It may not have been designed to have marginal gains over other selections, and may be selects sentences as standalone evidences. The motivation of the proposed approach is unclear, and warrants a separate point. There are minor typos (e.g. see Table 1 caption  "the recall improves recall "), which could be ignored for now.
\end{quote}
\begin{quote}
    Motivation: The authors mention "We choose the ReLU function specifically because the submodularity of the SCMM function requires non-negativity ". This is not a suitable reason to design experiments. The guarantees should follow from the function that empirically works best, the functions should not be designed to get some theoretical result and show it works "reasonably well" in practice. The "attention mechanism " motivation is very weak and does not justify the design or the greedy regularization. Why select a subset when the full problem can be tractably solved ? Again this could just be lazy writing. 
\end{quote}
\begin{quote}
    Empirical evaluation: One task and evaluation does not suggest that the proposed methodology is useful. Even ignoring the holes in writing, a single task and empirical evaluation on one dataset with precision/recall/F1 scores at different k is not evidence that the proposed method is verified. It does not even justify the title. Are there no other baselines that the proposed method could be compared against? This paper is not about "Differentiable Greedy Networks", it is about "greedy evidence selection for verifying claims using Recurrent NN". 
\end{quote}

\section{Rebuttal1}
Thanks for your feedback.  We provide here a pointwise response to your comments highlighting the changes we have made to the paper to address your concerns
\begin{itemize}
    \item "Writing: Needs major work. There are 3.5 pages of introduction and unnecessary background on submodular functions and two paragraphs in sec 3.2 of what the method proposed in this paper does. Only mentioning what the submodular function is, and may be a couple of references for it should have been enough....."
    
    We have reduced our background discussion on submodular functions. However we do feel that some introductory material is warranted to set the context for the rest of the paper.
    
    \item " The intro itself needs major revisions to be readable, there are a lot of holes. e.g. what is "unfolding" of the greedy algorithm that the  authors refer to Use of $\tau$ in f() should be explicitly written as an equation, so the reader doesn’t have to look at the paper by Jang et al to know that the exact expression is used in the training. "
    
    As recommended we have made the introduction easier to read.
    
    \item "What is  the DeepEncoder architecture? Why was it used as a baseline? Why cant diversity arguments not be made by easily altering the DeepEncoder cost function? It may not have been designed to have marginal gains over other selections, and may be selects sentences as standalone evidences. The motivation of the proposed approach is unclear, and warrants a separate point. There are minor typos (e.g. see Table 1 caption  "the recall improves recall "), which could be ignored for now."
    
    We have moved the description of the deep encoder to the experiment section and expanded on the definition and fixed the mentioned typos. We are not sure what you mean by the DeepEncoder cost function question, but since that model is a deep feedforward network, it considers each sentence independently, which we argue is a disadvantage since it does not account for redundancy.
    
    \item "The authors mention "We choose the ReLU function specifically because the submodularity of the SCMM function requires non-negativity ". This is not a suitable reason to design experiments. The guarantees should follow from the function that empirically works best, the functions should not be designed to get some theoretical result and show it works "reasonably well" in practice. The "attention mechanism " motivation is very weak and does not justify the design or the greedy regularization. Why select a subset when the full problem can be tractably solved? Again this could just be lazy writing. "
    
    The ReLU function is a important part of our algorithm design. We don't restrict baseline methods to be ReLU in order to compare. ReLU is known to be a non linearity of choice in many recent papers~\cite{}. The full problem cannot be tractably solved at scale since all subsets need to be considered and this can get prohibitively large. Furthermore, it would be both prohibitively expensive and counterproductive to use every sentence as evidence from a large dataset in a recognizing textual entailment task.
    
    \item "Empirical evaluation: One task and evaluation does not suggest that the proposed methodology is useful. Even ignoring the holes in writing, a single task and empirical evaluation on one dataset with precision/recall/F1 scores at different k is not evidence that the proposed method is verified. It does not even justify the title. Are there no other baselines that the proposed method could be compared against? This paper is not about "Differentiable Greedy Networks", it is about "greedy evidence selection for verifying claims using Recurrent NN". 
    
    Thank you for the feedback. Experimental results on diverse tasks will help to make our claims stronger.
    
\end{itemize}

\section{back1}
I find this comment a little frustrating. The reviewer deems the material they personally are presumably familiar with (submodularity) superfluous, and the unfamiliar material (unfolding) nonexistent. Some comments are not consistent: the definition of submodularity is unnecessary, but softmax temperature requires an equation. It seems like they just skipped section 2. 

That being said, I think it's best to prune some of the submodular section. By adding additional experiments with different submodular functions, we can focus less on the SCMM used for evidence retrieval and maybe remove some of the description, and even all of prop 1. We should probably briefly define unfolding in the intro, too. 

The sentences explaining the encoder and deep encoder baselines are present, but maybe it requires a little too much induction to infer the architecture--DGN has a dense feedforward layer + relu (i.e. the encoder) + shared greedy layers -> encoder is DGN minus the greedy part -> deep encoder has an extra dense layer. The answers to what and why of the deepencoder are in the second-to-last paragraph of page 6. 

I'm not really sure what to make of the comment ``Why cant diversity arguments not be made by easily altering the DeepEncoder cost function? It may not have been designed to have marginal gains over other selections, and may be selects sentences as standalone evidences.'' Is the reviewer answering their own question? Perhaps we didn't adequately justify our motivation for wanting to model dependencies between sentences.



Not sure why the reviewer latched on to this particular detail as the paper's motivation.


------------------------------------------------------------------------------------------------------------------------------------
------------------------------------------------------------------------------------------------------------------------------------

Reviewer 2 comments:

\begin{quote}
    The idea is incremental: it applies the greedy algorithm to the outputs of a Linear+ReLU layer, whose inputs are the pre-computed similarity scores. Unfolding the greedy algorithm produces a simple RNN with each unit computing the marginal gain conditioned on the previously selected elements (the previous state), but it does not increase the depth and thus does not improve representativeness. 
\end{quote}

\section{rebuttal2}
Thanks for your feedback.  We provide here a pointwise response to your comments highlighting the changes we have made to  address your concerns and make the paper better.
\begin{itemize}

\item "Unfolding the greedy algorithm produces a simple RNN with each unit computing the marginal gain conditioned on the previously selected elements (the previous state), but it does not increase the depth and thus does not improve representativeness."

The unfolding process is not sensitive to order like a RNN architecture. The proposed technique does not increase depth but is targeted towards better sentence selection via a submodular loss function.



\item "In addition, the idea of learning the weights in a submodular function has been studied in many previous works such as learning submodular mixture and deep submodular functions, and the idea can be applied to more general submodular functions rather than the specific one used in this paper. Hence, the contribution and novelty of this paper are very limited."
* Rasool will fill
 * Tommy can you list all differences between our works and previous ones 
 The difference between our approach and approaches like deep submodular functions is that we learn the parameters of a function through the optimization algorithm itself. Our approach can be applied to arbitrary submodular functions such as a deep submodular function \cite{BilmesB17}, not just the SCMM we used for our experiments because the point is that we are unfolding the inference algorithm, the forward greedy algorithm in this case, which itself can be used to optimize many different discrete functions. \citep{sipos2012} and \citep{tschiatschek2018differentiable} are more similar to our approach, though the model proposed by \citep{sipos2012} learns the weights of the function in a structured support vector machine framework, and the algorithms used by \citep{tschiatschek2018differentiable} rely on probabilistic algorithms.
 
\item    "During training, softmax is used to approximate argmax and make the computational graph differentiable. Why not using Gumbel-softmax (which was studied in the paper that the authors cited to support their use of softmax here), which is a better approximation of argmax? In addition, the differentiability comes from using softmax, but this makes the training not exactly optimizing for the original greedy algorithm but a soft version of it."
* We agree that in the general case Gumbel Softmax should help but for our particular data set with very few valid claims it didn't improve results. We found temperature annealing to be effective in addressing the concern regarding the use of argmax. Please refer to the new results in Table 3 of the updated paper.  

\item "None of any previous works has been compared in the experiments except baselines created by the authors. At least, attention-based models and RNN such as Transformer and LSTM should be compared, since the proposed model is similar to them on some main ideas: it can be explained as an attention mechanism using the marginal gain of the submodular function as the attention score function; and it can be also explained as an unfolded simple RNN."

    The main focus of this work is to introduce this new optimization scheme rather than focus on a complex model for sentence retrieval. More complex models such as Transformer can potentially improve the sentence selection itself but they don't address the problem of selecting the right \it{set} of sentences.

\item
\end{itemize}
\begin{quote}
    Since the transformation applied to the input similarity scores is linear, it might not be very helpful and the final performance might largely depend on the quality of the similarity metric used to compute the input scores. In addition, the idea of learning the weights in a submodular function has been studied in many previous works such as learning submodular mixture and deep submodular functions, and the idea can be applied to more general submodular functions rather than the specific one used in this paper. Hence, the contribution and novelty of this paper are very limited.
\end{quote}
 * Rasool will fill
 * Tommy can you list all differences between our works and previous ones 
 The difference between our approach and approaches like deep submodular functions is that we learn the parameters of a function through the optimization algorithm itself. Our approach can be applied to arbitrary submodular functions such as a deep submodular function \cite{BilmesB17}, not just the SCMM we used for our experiments because the point is that we are unfolding the inference algorithm, the forward greedy algorithm in this case, which itself can be used to optimize many different discrete functions. \citep{sipos2012} and \citep{tschiatschek2018differentiable} are more similar to our approach. The main difference are the model proposed by \citep{sipos2012} learns the weights of the function in a structured support vector machine framework, and the algorithms used by \citep{tschiatschek2018differentiable} rely on probabilistic algorithms.
  
\begin{quote}
    During training, softmax is used to approximate argmax and make the computational graph differentiable. Why not using Gumbel-softmax (which was studied in the paper that the authors cited to support their use of softmax here), which is a better approximation of argmax? In addition, the differentiability comes from using softmax, but this makes the training not exactly optimizing for the original greedy algorithm but a soft version of it.
\end{quote}
* In general we think Gumbel Softmax should help but for our particular data set with very few valid claims it did not improve results. We found temperature annealing to be effective in addressing the concern regarding the use of argmax. Please refer to the new results in Table 3 of the updated paper.  

Gumbel softmax adds ramdomness on forward pass, and is just a softmax on the backward. Also, yes, that is a necessary side effect of making it differentiable, and the reason we explored the effect of softmax temp. Maybe we should ``invent'' a new deterministic gubmel softmax (the hard-softmax, concrete softmax) rather than saying we use softmax on the backward pass and hard on the forward (only half-joking here).

\begin{quote}
    None of any previous works has been compared in the experiments except baselines created by the authors. At least, attention-based models and RNN such as Transformer and LSTM should be compared, since the proposed model is similar to them on some main ideas: it can be explained as an attention mechanism using the marginal gain of the submodular function as the attention score function; and it can be also explained as an unfolded simple RNN.
\end{quote}
    "The main focus of this work is to introduce this new optimization scheme rather than focus on a complex model for sentence retrieval. More complex models such as Transformer can potentially improve the sentence selection itself but they don't address the problem of selecting the right \it{set} of sentences."
    
\begin{quote}
    In experiments, the proposed DGN has the same performance or shows slight advantages when comparing to "Encoder", which does not use any greedy procedure at all. Does this suggest that the greedy procedure is not necessary?
\end{quote}
This is a point we need to address more thoroughly. We did try to address this with the last paragraph on page 7, and maybe we can make a stronger case for this with data that has more apparent diminishing returns.

\begin{quote}
    Proposition 1 had already been proved in classical submodular textbooks.
\end{quote}
Yes, we provided it for completeness. Given that both reviewers commented on this, we should probably explicitly say that this is known.

\begin{quote}
    Is the ground truth labels L in Eq.(5) a subset (as defined above the equation) or a subsequence (as indexed in the equation)? Which one provides better training signals?
\end{quote}


General notes: Many of the comments are rooted in the fact that we have one experiment with one submodular function. An additional exp would strengthen our argument that the unfolding greedy algorithms is broadly applicable.


------------------------------------------------------------------------------------------------------------------------------------
------------------------------------------------------------------------------------------------------------------------------------
Reviewer 3 comments:

Problems: 
* While the paper seems to be well motivated, some of the claims are
justified in a hand-waving manner and could be better justified with either a
more theoretical exposition or empirical analysis. For eg., the utility of ReLU,
while the theoretical justification is clear, how important was the
non-linearity in the entire scheme of DGN? Or the relation to attention
architectures - while the proposed method is superior to simple attentional architectures 
can this be related to decomposable attention [1] or the hierarchical attention architecture[2]?

* Ablation between different families of claims: I suppose the submodular
function is going to be very useful when the number of evidences are more than
two. The paper could have benefitted from ablation between different types of
claims: claims with one/two sentence as evidence vs claims with more than two
sentences as evidences.

* The claim that greedy DGN outperforming conventional discrete opitmization
  algorithms is strong given sparse comparisons to conventional techniques. 
  
** Top-K and Greedy in Table 1 cover baseline discrete optimizations that we compared against.
Questions:

* From the experiments in the paper it seems like the temperature is
  a very delicate hyperparameter and the range from $(3, 6)$ seems like the
  function is not close to argmax. Would this mean that the trained model is
  suboptimal? I would also suggest the authors to kindly add the ablations of
  temperature (with annealing) to the appendix. 

* The descriptions of encoder and deepencoder are very confusing. Is the only
  addition to the deep encoder is an additional non-linear layer? In any case,
  Table 2 suggests the deep encoder performs comparably to DGN, apart from the
  problems with class imbalance, given its performance, is it correct to say
  that deepencoder learns robust representations? In other words, the advantages
  of DGN are still not clear. Is the greedy algorithm helping in selecting the
  k sentences? If so, how many of the cases have k>2 and was DGN better there? 

* What happens when the similarity is computed using say euclidean distance?
  How would the temperature hyperparameter change?



Other Issues: 
* The sections in paper need rewriting, especially section 4. 

* Comparisons: it would have been ideal to have the comparisons to attention
  based approaches (simple attention, hierarchical attention) with standard
  optimization techniques. 


[1] Parikh, Ankur P., et al. "A decomposable attention model for natural language inference." arXiv preprint arXiv:1606.01933 (2016).
[2] Yang, Zichao, et al. "Hierarchical attention networks for document classification." Proceedings of the 2016 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies. 2016.

\section{Rebuttal3}
**THIS IS VERY INCOMPLETE. WE RAN OUT OF TIME DISCUSSING REVIEWER3 

Thanks for your feedback.  We provide here a pointwise response to your comments highlighting the changes we have made to  address your concerns and make the paper better.

\begin{itemize}
    \item While the paper seems to be well motivated, some of the claims are
justified in a hand-waving manner and could be better justified with either a
more theoretical exposition or empirical analysis. For eg., the utility of ReLU,
while the theoretical justification is clear, how important was the
non-linearity in the entire scheme of DGN? Or the relation to attention
architectures - while the proposed method is superior to simple attentional architectures can this be related to decomposable attention [1] or the hierarchical attention architecture[2]?

    \item The claim that greedy DGN outperforming conventional discrete optimization
  algorithms is strong given sparse comparisons to conventional techniques. 
  
** Top-K and Greedy in Table 1 cover baseline discrete optimizations that we compared against.
Questions:
   \item
\end{itemize}


